Smallest Multiplicative Stretch for an $\alpha$-APASP Below $\widetilde O \left(n^{\omega}\right)$ Runtime

Dor, Halperin and Zwick [FOCS'96; SICOMP'00] showed that $(2-\varepsilon)$-APASP is at least as hard as BMM for every fixed $0<\varepsilon<1$. Zwick [FOCS'98; JACM'02] gave a $2$-APASP algorithm in $\widetilde O(n^{\omega+o(1)}\log W_{\max})$ runtime, where $W_{\max}$ is the maximum edge weight. Bringmann, K{\"u}nnemann and W{\k{e}}grzycki [STOC'19] removed this logarithmic factor. Using OpenAI's recent bound $\omega\leq\frac{9}{4}$ gives $\widetilde O\left(n^{\frac{9}{4}+o(1)}\right)$ time. We present two weighted undirected $2$-APASP algorithms. The first uses $(\min,\max)$-products. Earlier rectangular FMM bounds of Vassilevska Williams, Yinzhan Xu, Zixuan Xu and Zhou [SODA'24] and Alman, Duan, Vassilevska Williams, Yinzhan Xu, Zixuan Xu and Zhou [SODA'25] give $\widetilde O(n^{2.36999465})$ runtime, below the previous $\omega\leq2.371177$ of Dupont, Eisenberger, Kozlovskii, Mehrabian, Ruiz, See, Zhou, Alman, Vassilevska Williams and Balog [arXiv'26]. Current rectangular FMM bounds give $\widetilde O(n^{2.34549151})$, independent of $W_{\max}$. For integer weights, our second algorithm has $\widetilde O(n^{\omega-\frac{(\omega-2)^2}{\omega-1}+o(1)}\log^{O(1)}W_{\max})$ runtime, with exponent below $\omega$ whenever $\omega>2$. The rectangular bounds of Uzna{\'n}ski [arXiv'26] or of Amanov, van den Berg and Zuiddam [arXiv'26] give $\widetilde O(n^{2.17157288}\log^{O(1)}W_{\max})$.

==> Illustrations/APASP/caseTree.tex <==
\usetikzlibrary{positioning,calc}

\begin{tikzpicture}[
  >=latex,
  every node/.style={
    font=\small,
    align=center
  },
  branch/.style={
    line width=0.8pt
  },
  caselabel/.style={
    font=\small,
    align=center,
    fill=white,
    inner sep=2pt
  },
  linelabel/.style={
    font=\small,
    align=center,
    fill=white,
    inner xsep=3pt,
    inner ysep=1pt
  },
  condition/.style={
    font=\small,
    align=center,
    text width=3.2cm,
    inner sep=2pt
  },
  action/.style={
    text width=3.2cm,
    align=center,
    inner sep=2pt
  },
  smallaction/.style={
    text width=2.8cm,
    align=center,
    inner sep=2pt
  }
]

% ============================================================
% 1. TOP LEVEL
% ============================================================

\node (B2) {$B_2(u), B_2(v)$};

\coordinate (topLevel)
  at ([yshift=-1.5cm]B2.center);

\coordinate (topDisjoint)
  at ([xshift=-5.8cm]topLevel);

\coordinate (topTouch)
  at (topLevel);

\coordinate (topOverlap)
  at ([xshift=5.8cm]topLevel);


\draw[branch]
  (B2.south) -- (topLevel);

\draw[branch]
  (topDisjoint) -- (topOverlap);


% Give the top labels a little more breathing room
\node[caselabel, above=5pt of topDisjoint]
  {Disjoint};

\node[caselabel, above=5pt of topTouch]
  {Touch at edge $(x,y)$};

\node[caselabel, above=5pt of topOverlap]
  {Overlap};


% ============================================================
% 2. DISJOINT BRANCH
% ============================================================

\node[action] (reportS2)
  at ([yshift=-2.0cm]topDisjoint)
  {
    % Report $d(u,v)$ through\\
    % $p_2(u),p_2(v)$\\
    % $(2\text{-Approx.})$
    Lines \ref{algline:2-APASP-slower-main-pivotMSSP}-\ref{algline:2-APASP-slower-main-pivotUpdate}\\
    (for $i=3$)
  };

\draw[branch]
  (topDisjoint) -- (reportS2.north);


\node (costS2)
  [below=4mm of reportS2]
  {
    $\bigl(n^{1-a-b}\bigr)\bigl(n^2\bigr)$
  };


% ============================================================
% 3. TOUCH BRANCH
% ============================================================

\node (checkB1Touch)
  at ([yshift=-2.05cm]topTouch)
  {
    Check $B_1(x), B_1(y)$
  };


\draw[branch]
  (topTouch) -- (checkB1Touch.north);


% Place the label BESIDE the line rather than on it
\coordinate (notE2pos)
  at ($(topTouch)!0.50!(checkB1Touch.north)$);

\node[linelabel, left=1mm of notE2pos]
  {$(x,y)\notin E_2$};


% ============================================================
% 4. TOUCH SPLIT
% ============================================================

\coordinate (touchSplit)
  at ([yshift=-1.25cm]checkB1Touch.center);

\coordinate (touchBadPoint)
  at ([xshift=-2.7cm]touchSplit);

\coordinate (touchGoodPoint)
  at ([xshift=2.7cm]touchSplit);


\draw[branch]
  (checkB1Touch.south) -- (touchSplit);

\draw[branch]
  (touchBadPoint) -- (touchGoodPoint);


% ============================================================
% 5. CONDITION NODES
%
% Important change:
% the lines terminate at the text rather than running through it.
% ============================================================

\node[
  condition,
  below=5mm of touchBadPoint
] (touchBadCondition)
  {
    $u\notin B_1(x)$ or\\
    $v\notin B_1(y)$
  };


\node[
  condition,
  below=5mm of touchGoodPoint
] (touchGoodCondition)
  {
    $u\in B_1(x)$ and\\
    $v\in B_1(y)$
  };


\draw[branch]
  (touchBadPoint)
  -- (touchBadCondition.north);

\draw[branch]
  (touchGoodPoint)
  -- (touchGoodCondition.north);


% ============================================================
% 6. BAD TOUCH CASE
% ============================================================

\node[action] (reportMinMax)
  [below=9mm of touchBadCondition]
  {
    % Report through $(\min,\max)$\\[1mm]
    % $\displaystyle
    %   n^{\frac{3-a+\omega(1,1-a,1)}{2}}
    % $\\
    % $(2\text{-Approx.})$
    Lines \ref{algline:2-APASP-slower-main-pivotMSSP} (for $i=2$),\\ 
    \ref{algline:2-APASP-slower-main-distanceUpdate-start}-\ref{algline:2-APASP-slower-main-distanceUpdate-end}, \ref{algline:2-APASP-slower-main-pivotMSSP-again}, \ref{algline:2-APASP-slower-main-minmax-update}
  };


\draw[branch]
  (touchBadCondition.south)
  -- (reportMinMax.north);


% ============================================================
% 7. OVERLAP BRANCH
% ============================================================

\node[smallaction] (sampleBig)
  at ([yshift=-2.05cm]topOverlap)
  {
    Sample to\\
    $n^{1+a+b}$ edges
  };


\draw[branch]
  (topOverlap)
  -- (sampleBig.north);


% ============================================================
% 8. TOUCH CASE WITH (x,y) in E_2
% ============================================================

% Give this connector its own horizontal corridor

\coordinate (E2start)
  at ([yshift=-0.65cm]topTouch);

\coordinate (E2turn)
  at ([xshift=2.2cm]E2start);

\coordinate (E2right)
  at (sampleBig.north |- E2turn);


\draw[branch]
  (topTouch)
  -- (E2start)
  -- (E2right)
  -- (sampleBig.north);


% Put text ABOVE the line, with white background
\coordinate (E2labelpos)
  at ($(E2turn)!0.55!(E2right)$);

\node[
  linelabel,
  above=-5pt of E2labelpos
]
  {$(x,y)\in E_2$};


% ============================================================
% 9. OVERLAP CHECK
%
% This is deliberately moved lower than before.
% That separates it from the touch-condition text.
% ============================================================

\node (checkB1Overlap)
  [below=16mm of sampleBig]
  {
    Check $B_1(u), B_1(v)$
  };


\draw[branch]
  (sampleBig.south)
  -- (checkB1Overlap.north);


% ============================================================
% 10. OVERLAP SPLIT
% ============================================================

\coordinate (overlapSplit)
  at ([yshift=-1.25cm]checkB1Overlap.center);

\coordinate (overlapGoodPoint)
  at ([xshift=-1.8cm]overlapSplit);

\coordinate (overlapBadPoint)
  at ([xshift=1.8cm]overlapSplit);


\draw[branch]
  (checkB1Overlap.south)
  -- (overlapSplit);

\draw[branch]
  (overlapGoodPoint)
  -- (overlapBadPoint);


% ============================================================
% 11. OVERLAP CONDITION NODES
% ============================================================

\node[
  condition,
  text width=2.5cm,
  below=5mm of overlapGoodPoint
] (overlapGoodCondition)
  {
    Touch/\\
    Overlap
  };


\node[
  condition,
  text width=2.5cm,
  below=5mm of overlapBadPoint
] (overlapBadCondition)
  {
    Disjoint
  };


\draw[branch]
  (overlapGoodPoint)
  -- (overlapGoodCondition.north);

\draw[branch]
  (overlapBadPoint)
  -- (overlapBadCondition.north);


% ============================================================
% 12. OVERLAP -> DISJOINT
% ============================================================

\node[action] (reportS1)
  [below=9mm of overlapBadCondition]
  {
    % Report $d(u,v)$ through\\
    % $p_1(u),p_1(v)$\\
    % $(2\text{-Approx.})$
    Lines \ref{algline:2-APASP-slower-main-pivotMSSP}-\ref{algline:2-APASP-slower-main-pivotUpdate}\\
    (for $i=2$)
  };


\draw[branch]
  (overlapBadCondition.south)
  -- (reportS1.north);


\node (costS1)
  [below=4mm of reportS1]
  {
    $\bigl(n^{1-a}\bigr)
     \bigl(n^{1+a+b}\bigr)$
  };


% ============================================================
% 13. SHARED GOOD-BRANCH CONTINUATION
% ============================================================

% Drop each successful branch below its label FIRST.
% This prevents vertical lines from crossing the text.

\coordinate (touchGoodDown)
  at ([yshift=-1.15cm]touchGoodCondition.south);

\coordinate (overlapGoodDown)
  at ([yshift=-1.15cm]overlapGoodCondition.south);


% Shared join x-position
\coordinate (joinX)
  at ($(touchGoodCondition)!0.55!(overlapGoodCondition)$);


% Keep join comfortably below both branches
\coordinate (joinLevel)
  at ([yshift=-1.15cm]overlapGoodCondition.south);

\coordinate (join)
  at (joinX |- joinLevel);


% Touch-good route
\draw[branch]
  (touchGoodCondition.south)
  -- (touchGoodDown)
  |- (join);


% Overlap-good route
\draw[branch]
  (overlapGoodCondition.south)
  -- (overlapGoodDown)
  |- (join);


% ============================================================
% 14. FINAL SHARED CHAIN
% ============================================================

\node[smallaction] (sampleSmall)
  [below=9mm of join]
  {
    Sample to\\
    $n^{1+a}$ edges
  };


\node[smallaction] (exact)
  [below=9mm of sampleSmall]
  {
    % Exact APSP\\
    % $+$ edge-disjoint updates
    Line \ref{algline:2-APASP-slower-main-estimateAPSP}
  };


\node (optimal)
  [below=4mm of exact]
  {
    $n\bigl(n^{1+a}\bigr)$\\[-1mm]
    % $(\text{optimal})$
  };


\draw[branch]
  (join)
  -- (sampleSmall.north);

\draw[branch]
  (sampleSmall.south)
  -- (exact.north);

% \draw[branch]
%   (exact.south)
%   -- (optimal.north);

\end{tikzpicture}

==> Illustrations/APASP/caseTree_new.tex <==
\usetikzlibrary{positioning,calc}

\begin{tikzpicture}[
  >=latex,
  every node/.style={
    font=\small,
    align=center
  },
  branch/.style={
    line width=0.8pt
  },
  caselabel/.style={
    font=\small,
    align=center,
    fill=white,
    inner sep=2pt
  },
  linelabel/.style={
    font=\small,
    align=center,
    fill=white,
    inner xsep=3pt,
    inner ysep=1pt
  },
  condition/.style={
    font=\small,
    align=center,
    text width=3.0cm,
    inner sep=2pt
  },
  action/.style={
    text width=3.2cm,
    align=center,
    inner sep=2pt
  },
  smallaction/.style={
    text width=2.7cm,
    align=center,
    inner sep=2pt
  }
]

% ============================================================
% 1. TOP LEVEL
% ============================================================

\node (title)
{
  Value of $|E(P)\setminus E_3|$
  (Assume $P$ is $(u,v)$-shortest path)
};

\coordinate (topLevel)
  at ([yshift=-1.35cm]title.center);

\coordinate (topMany)
  at ([xshift=-6.0cm]topLevel);

\coordinate (topOne)
  at ([xshift=-1.4cm]topLevel);

% Shifted right from 4.3cm to 5.3cm.
% The entire |E(P)\setminus E_3|=0 subtree moves with this.
\coordinate (topZero)
  at ([xshift=5.3cm]topLevel);


\draw[branch]
  (title.south) -- (topLevel);

\draw[branch]
  (topMany) -- (topZero);


\node[caselabel, above=5pt of topMany]
{
  $|E(P)\setminus E_3|\ge 2$
};

\node[caselabel, above=5pt of topOne]
{
  $|E(P)\setminus E_3|=1$
  $(P=u\leadsto x-y\leadsto v)$
};

\node[caselabel, above=5pt of topZero]
{
  $|E(P)\setminus E_3|=0$
};


% ============================================================
% 2. |E(P) \ E_3| >= 2
% ============================================================

\node[action] (reportP2)
  at ([yshift=-2.20cm]topMany)
{
  Dijkstra for $S_3$ over $E$. Then report $d[u,v]$
  through $p_3(u),p_3(v)$.\\
  (Gives 2-Approx.)
};

\draw[branch]
  (topMany) -- (reportP2.north);


\node (costP2)
  [below=6mm of reportP2]
{
  Lines \ref{algline:2-APASP-faster-main-pivotMSSP}-\ref{algline:2-APASP-faster-main-pivotUpdate} (for $i=4$)\\
  $\bigl(n^{1-a-b-c}\bigr)\bigl(n^2\bigr)$
};


% ============================================================
% 3. |E(P) \ E_3| = 1
% ============================================================

\node[
  condition,
  text width=4cm
] (notE3)
  at ([yshift=-2.55cm]topOne)
{
  Note $(x,y)\notin E_3$. \\
  Hence, $(x,y) \notin E_2$.
};


\draw[branch]
  (topOne)
  -- (notE3.north);


\node (checkB1xy)
  [below=15mm of notE3]
{
  Check $B_2(x), B_2(y)$
};


\draw[branch]
  (notE3.south)
  -- (checkB1xy.north);


% ============================================================
% 4. CHILDREN OF Check B_2(x), B_2(y)
% ============================================================

\coordinate (xyDrop)
  at ([yshift=-1.10cm]checkB1xy.south);

\coordinate (xySplit)
  at ([xshift=-2.40cm]xyDrop);

\coordinate (xyBadPoint)
  at ([xshift=-2.15cm]xySplit);

\coordinate (xyGoodPoint)
  at ([xshift=4.15cm]xySplit);


\draw[branch]
  (checkB1xy.south)
  -- (xyDrop)
  -- (xySplit);

\draw[branch]
  (xyBadPoint)
  -- (xyGoodPoint);


% ============================================================
% 5. CHILD CONDITIONS OF Check B_2(x), B_2(y)
% ============================================================

\node[
  condition,
  below=7mm of xyBadPoint
] (xyBadCondition)
{
  $u\notin B_2(x)$ or\\
  $v\notin B_2(y)$
};


\node[
  condition,
  below=7mm of xyGoodPoint
] (xyGoodCondition)
{
  $u\in B_2(x)$ and\\
  $v\in B_2(y)$.\\
%   This implies
%   $\delta(u,x), \delta(y,v) \leq w(x,y)$.\\

  Assume $\delta(u,x) \leq \delta(y,v)\leq w(x,y)$.
};


\draw[branch]
  (xyBadPoint)
  -- (xyBadCondition.north);

\draw[branch]
  (xyGoodPoint)
  -- (xyGoodCondition.north);


% ============================================================
% 6. BAD CHILD OF Check B_2(x), B_2(y)
% ============================================================

\node[action] (reportMinMax)
  [below=13mm of xyBadCondition, text width=4cm]
{
  Dijkstra for $S_2$ over $E_3$.
  Then pivot distance updates for all pairs.
  Then Dijkstra for $S_2$ over $E_3$ again.

  \vspace{5mm}
  Lines \ref{algline:2-APASP-slower-main-pivotMSSP} (for $i=3$), \ref{algline:2-APASP-slower-main-distanceUpdate-start}-\ref{algline:2-APASP-slower-main-distanceUpdate-end}, \ref{algline:2-APASP-slower-main-pivotMSSP-again} \\
  $\bigl(n^{1-a-b}\bigr)\bigl(n^{1+a+b+c}\bigr)$
  \vspace{4mm}

  Then report through $(\min,\max)$ of $V \times S_2$.\\
  (Gives 2-Approx.)

};


\node (costreportMinMax)
  [below=6mm of reportMinMax]
{
  Line \ref{algline:2-APASP-faster-main-minmax-update} \\
  $\bigl(n^{\frac{3-a-b+\omega(1,1-a-b,1)}{2}}\bigr)$
};


\draw[branch]
  (xyBadCondition.south)
  -- (reportMinMax.north);


% ============================================================
% 7. GOOD CHILD OF Check B_2(x), B_2(y)
% ============================================================

\node[smallaction] (sampleXYGood)
  [below=13mm of xyGoodCondition, text width=4cm]
{
  Value of $|E(P)\setminus E_1|$
};


\draw[branch]
  (xyGoodCondition.south)
  -- (sampleXYGood.north);


% ============================================================
% 7A. TWO BRANCHES OF
%     "Check |E(P) \ E_1| value."
% ============================================================

\coordinate (xyGoodChildSplit)
  at ([yshift=-1.10cm]sampleXYGood.south);

\coordinate (xyGoodChildLeftPoint)
  at ([xshift=-1.85cm]xyGoodChildSplit);

\coordinate (xyGoodChildRightPoint)
  at ([xshift=1.85cm]xyGoodChildSplit);


% Stem from parent
\draw[branch]
  (sampleXYGood.south)
  -- (xyGoodChildSplit);

% Horizontal sibling bar
\draw[branch]
  (xyGoodChildLeftPoint)
  -- (xyGoodChildRightPoint);


% Branch labels
\node[
  caselabel,
  above=5pt of xyGoodChildLeftPoint,
  xshift=4mm
]
{
  $|E(P)\setminus E_1|=1$
};


\node[
  caselabel,
  above=5pt of xyGoodChildRightPoint
]
{
  $|E(P)\setminus E_1| \geq 2$
};


% ============================================================
% LEFT CHILD: |E(P) \ E_1| = 1
% ============================================================

\node[action] (dijkstraXYGoodLeft)
  [below=10mm of xyGoodChildLeftPoint]
{
  Run Dijkstra for APSP
  twice on $E_1$.\\
  Gives exact
  distance.
};


\draw[branch]
  (xyGoodChildLeftPoint)
  -- (dijkstraXYGoodLeft.north);


\node (costXYGoodLeft)
  [below=6mm of dijkstraXYGoodLeft]
{
  Line \ref{algline:2-APASP-faster-main-estimateAPSP} \\
  $\bigl(n\bigr)\bigl(n^{1+a}\bigr)$
};


% ============================================================
% RIGHT CHILD: |E(P) \ E_1| >= 2
% ============================================================

\node[action] (dijkstraXYGoodRight)
  [below=10mm of xyGoodChildRightPoint]
{
  Check $B_1(u)$
};


\draw[branch]
  (xyGoodChildRightPoint)
  -- (dijkstraXYGoodRight.north);


% ============================================================
% CHILDREN OF Value of |E(u \squiggly x) \ E_1|
% ============================================================

\coordinate (uxE1Split)
  at ([yshift=-0.65cm]dijkstraXYGoodRight.south);

\coordinate (uxE1ZeroPoint)
  at ([xshift=-1.25cm]uxE1Split);

\coordinate (uxE1ManyPoint)
  at ([xshift=5cm, yshift=3cm]uxE1Split);


% Stem from parent
\draw[branch]
  (dijkstraXYGoodRight)
  -- (uxE1ManyPoint);

% Horizontal sibling bar
\draw[branch]
  (uxE1ZeroPoint)
  -- (dijkstraXYGoodRight.south);


% Left child
\node[
  condition,
  text width=4cm,
  below=6mm of uxE1ZeroPoint
] (uxE1Zero)
{
  $x \notin B_1(u)$\\

  \vspace{2mm}

  This implies $\delta(u, p_1(u)) \leq \frac{\delta(u,v)}{3}$.
  Do approximate MSSP over $S_1$ and then approx. $(min, +)$ for $V \times S_1$. 
  (Gives $(\frac{5}{3} + \epsilon)$-approximation)

  \vspace{4mm}
  
  Lines \ref{algline:2-APASP-faster-main-approxMSSP}-\ref{algline:2-APASP-faster-main-pivot-approxMinPlus-end} \\
  $\bigl(n^{\omega(1,1-a,1)}\bigr)$.

};


% Right child
\node[
  condition,
  text width=7cm,
  below=6mm of uxE1ManyPoint
] (uxE1Many)
{
  $x \in B_1(u)$\\

  \vspace{2mm}

  $P = u \squiggly x - y \squiggly x' - y' \squiggly v$ \\
  $u \squiggly x \in E_1, \ (x,y) \notin E_1$ \\
  Let $w(x,y) = W$, note $\delta(y, v) \leq W$.\\
  For any $(x', y') \in y \squiggly v$ such that $(x', y') \notin E_1$, we can assume that $\delta(x', p_1(x')) \geq \frac{7}{8}W$, otherwise approx. MSSP, $(min, +)$ from $p_1(x')$ already give 2-Approx. As $w(x', y') \geq \delta(x', p_1(x'))$, this implies $W \geq w(x', y') \geq \frac{7}{8}W$. \\
  So, for every vertex $h \in u \squiggly v$, we have that $\delta(h, p_1(h)) \geq \frac{5}{6}W$, else approx. MSSP, $(min, +)$ from $p_1(h)$ already give 2 approx.\\ 

  Since $\delta(y, v) \leq W$, there can be at most 1 such edge $(x', y')$ in $y \squiggly v$. Also, $w(y \squiggly x'), w(y' \squiggly v) \leq \frac{1}{8}W$. This means $x' \in B_1(y), y \in B_1(x'), y' \in B_1(v), v \in B_1(y')$\\
  Hence, at most 2 edges of $P$ dont lie in $E_1$. 
%   So run Dijkstra for APSP 10 times on $E_1$. Gives exact distance.
  {\textbf{LS:} Dont know what to do here}
%   $n(n^{1+a})$

  
};


\draw[branch]
  (uxE1ZeroPoint)
  -- (uxE1Zero.north);

\draw[branch]
  (uxE1ManyPoint)
  -- (uxE1Many.north);



% ============================================================
% 9. VALUE OF |E(P) \ E_2|
% ============================================================

\node (valueE1)
  [below=11mm of topZero]
{
  Value of $|E(P)\setminus E_2|$
};


\draw[branch]
  (topZero.south)
  -- (valueE1.north);


% ============================================================
% 10. THREE-WAY SPLIT FOR |E(P) \ E_2|
% ============================================================

\coordinate (E1split)
  at ([yshift=-1.35cm]valueE1.south);

\coordinate (E1onePoint)
  at ([xshift=-2.65cm]E1split);

\coordinate (E1zeroPoint)
  at ([xshift=0.15cm]E1split);

\coordinate (E1manyPoint)
  at ([xshift=3.15cm]E1split);


\draw[branch]
  (valueE1.south)
  -- (E1split);

\draw[branch]
  (E1onePoint)
  -- (E1manyPoint);


% ============================================================
% 11. THREE CONDITIONS UNDER |E(P) \ E_2|
% ============================================================

\node[
  condition,
  text width=2.45cm,
  below=7mm of E1onePoint
] (E1one)
{
  $|E(P)\setminus E_2|=1$
};


\node[
  condition,
  text width=2.45cm,
  below=7mm of E1zeroPoint
] (E1zero)
{
  $|E(P)\setminus E_2|=0$
};


\node[
  condition,
  text width=2.55cm,
  below=7mm of E1manyPoint
] (E1many)
{
  $|E(P)\setminus E_2|\ge 2$
};


\draw[branch]
  (E1onePoint)
  -- (E1one.north);

\draw[branch]
  (E1zeroPoint)
  -- (E1zero.north);

\draw[branch]
  (E1manyPoint)
  -- (E1many.north);


% ============================================================
% 12. |E(P) \ E_2| = 1
%
% Redirect this case to Check B_2(x), B_2(y).
% ============================================================

\draw[
  branch,
  ->
]
  (E1one.west)
  -- ([xshift=0mm, yshift=1mm]checkB1xy.east);


% ============================================================
% 13. |E(P) \ E_2| = 0
% ============================================================



\node[action] (apspE1Zero)
  [below=11mm of E1zero]
{
  2-Approx APSP  over $E_2$.\\
  (Gives 2-Approx.)
};


\draw[branch]
  (E1zero.south)
  -- (apspE1Zero.north);


\node (costE1Zero)
  [below=6mm of apspE1Zero]
{
  Line \ref{algline:2-APASP-faster-main-BasKav-G2}\\
  $\bigl(n^{0.5}\bigr)\bigl(n^{1+a+b}\bigr)$
};


% ============================================================
% 14. |E(P) \ E_2| >= 2
% ============================================================

\node[action] (reportP1)
  [below=14mm of E1many]
{
  Dijkstra for $S_2$ over $E_3$. Then report $d[u,v]$
  through $p_2(u),p_2(v)$.\\
  (Gives 2-Approx.)
};


\draw[branch]
  (E1many.south)
  -- (reportP1.north);


\node (costP1)
  [below=6mm of reportP1]
{
  Lines \ref{algline:2-APASP-faster-main-pivotMSSP}-\ref{algline:2-APASP-faster-main-pivotUpdate} (for $i=3$)\\
  $\bigl(n^{1-a-b}\bigr) \bigl(n^{1+a+b+c}\bigr)$
};


\end{tikzpicture}

Important values to remember:
$$|S_1| = n^{1-a}, |S_2| = n^{1-a-b}, |S_3| = n^{1-a-b-c},
|E_1| = n^{1+a}, |E_2| = n^{1+a+b}, |E_3| = n^{1+a+b+c}$$

Also, $S_3 \subseteq S_2 \subseteq S_1 \subseteq V$
and
$E_1 \subseteq E_2 \subseteq E_3 \subseteq E$.

==> Illustrations/Balls/ballexample.tex <==
\begin{figure}[H]
\centering

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Ellipse [id:dp6625860162276211] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=0.55 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.29 ] (301.45,234.55) .. controls (272.97,209.21) and (270.06,166) .. (294.94,138.04) .. controls (319.82,110.09) and (363.07,107.97) .. (391.55,133.32) .. controls (420.03,158.67) and (422.94,201.87) .. (398.06,229.83) .. controls (373.18,257.78) and (329.93,259.9) .. (301.45,234.55) -- cycle ;
%Straight Lines [id:da9412047664314018] 
\draw    (314.73,189.53) -- (361.23,162.53) ;
%Straight Lines [id:da5938656329561427] 
\draw    (314.73,189.53) -- (358.73,226.2) ;
%Straight Lines [id:da15591646157325867] 
\draw    (358.73,226.2) -- (400.75,264) ;
%Straight Lines [id:da8588636129532099] 
\draw    (358.73,226.2) -- (434.75,226.5) ;
%Straight Lines [id:da3423424168072611] 
\draw    (400.75,264) -- (434.75,226.5) ;
%Straight Lines [id:da7252060609228765] 
\draw    (359.73,225.2) -- (434.25,164) ;
%Straight Lines [id:da8370853051570586] 
\draw    (434.25,164) -- (434.75,222.5) ;
%Straight Lines [id:da23613900566954826] 
\draw    (435.5,165.33) -- (471.75,201) ;
%Straight Lines [id:da18676055033971273] 
\draw    (438.25,162) -- (472.25,147) ;
%Straight Lines [id:da2707706875989797] 
\draw    (472.25,143) -- (472,110.67) ;
%Straight Lines [id:da8302620780031216] 
\draw    (364.23,160.53) -- (468.57,112.87) ;
%Straight Lines [id:da8037223017346966] 
\draw    (365.23,162.53) -- (434.25,163) ;
%Shape: Circle [id:dp40608497322126125] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (357.23,162.53) .. controls (357.23,160.32) and (359.02,158.53) .. (361.23,158.53) .. controls (363.44,158.53) and (365.23,160.32) .. (365.23,162.53) .. controls (365.23,164.74) and (363.44,166.53) .. (361.23,166.53) .. controls (359.02,166.53) and (357.23,164.74) .. (357.23,162.53) -- cycle ;
%Shape: Circle [id:dp26827319251987447] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (354.73,226.2) .. controls (354.73,223.99) and (356.52,222.2) .. (358.73,222.2) .. controls (360.94,222.2) and (362.73,223.99) .. (362.73,226.2) .. controls (362.73,228.41) and (360.94,230.2) .. (358.73,230.2) .. controls (356.52,230.2) and (354.73,228.41) .. (354.73,226.2) -- cycle ;
%Straight Lines [id:da8476855593267647] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (500.25,180) -- (477.58,154.49) ;
\draw [shift={(476.25,153)}, rotate = 48.37] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Circle [id:dp9709647852196648] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (310.73,189.53) .. controls (310.73,187.32) and (312.52,185.53) .. (314.73,185.53) .. controls (316.94,185.53) and (318.73,187.32) .. (318.73,189.53) .. controls (318.73,191.74) and (316.94,193.53) .. (314.73,193.53) .. controls (312.52,193.53) and (310.73,191.74) .. (310.73,189.53) -- cycle ;
%Shape: Circle [id:dp5706248374556] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (430.25,163) .. controls (430.25,160.79) and (432.04,159) .. (434.25,159) .. controls (436.46,159) and (438.25,160.79) .. (438.25,163) .. controls (438.25,165.21) and (436.46,167) .. (434.25,167) .. controls (432.04,167) and (430.25,165.21) .. (430.25,163) -- cycle ;
%Shape: Circle [id:dp6661137907917287] 
\draw  [color={rgb, 255:red, 126; green, 211; blue, 33 }  ,draw opacity=1 ][fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (468,110.67) .. controls (468,108.46) and (469.79,106.67) .. (472,106.67) .. controls (474.21,106.67) and (476,108.46) .. (476,110.67) .. controls (476,112.88) and (474.21,114.67) .. (472,114.67) .. controls (469.79,114.67) and (468,112.88) .. (468,110.67) -- cycle ;
%Shape: Circle [id:dp1158857638153572] 
\draw  [color={rgb, 255:red, 126; green, 211; blue, 33 }  ,draw opacity=1 ][fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (468.25,147) .. controls (468.25,144.79) and (470.04,143) .. (472.25,143) .. controls (474.46,143) and (476.25,144.79) .. (476.25,147) .. controls (476.25,149.21) and (474.46,151) .. (472.25,151) .. controls (470.04,151) and (468.25,149.21) .. (468.25,147) -- cycle ;
%Shape: Circle [id:dp7673589811197465] 
\draw  [color={rgb, 255:red, 126; green, 211; blue, 33 }  ,draw opacity=1 ][fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (467.75,201) .. controls (467.75,198.79) and (469.54,197) .. (471.75,197) .. controls (473.96,197) and (475.75,198.79) .. (475.75,201) .. controls (475.75,203.21) and (473.96,205) .. (471.75,205) .. controls (469.54,205) and (467.75,203.21) .. (467.75,201) -- cycle ;
%Shape: Circle [id:dp5265818224073935] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (430.75,226.5) .. controls (430.75,224.29) and (432.54,222.5) .. (434.75,222.5) .. controls (436.96,222.5) and (438.75,224.29) .. (438.75,226.5) .. controls (438.75,228.71) and (436.96,230.5) .. (434.75,230.5) .. controls (432.54,230.5) and (430.75,228.71) .. (430.75,226.5) -- cycle ;
%Shape: Circle [id:dp603509841517055] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (396.75,264) .. controls (396.75,261.79) and (398.54,260) .. (400.75,260) .. controls (402.96,260) and (404.75,261.79) .. (404.75,264) .. controls (404.75,266.21) and (402.96,268) .. (400.75,268) .. controls (398.54,268) and (396.75,266.21) .. (396.75,264) -- cycle ;

% Text Node
\draw (383.42,264.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle a_{3}$};
% Text Node
\draw (339.92,226.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle a_{2}$};
% Text Node
\draw (441.83,219.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle b_{2}$};
% Text Node
\draw (418,144) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle b_{1}$};
% Text Node
\draw (479.08,196.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 126; green, 211; blue, 33 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle s_{1}$};
% Text Node
\draw (479.08,107.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 126; green, 211; blue, 33 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle s_{3}$};
% Text Node
\draw (479.25,142.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 126; green, 211; blue, 33 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle s_{2}$};
% Text Node
\draw (357.25,169.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle u$};
% Text Node
\draw (394,213) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 1$};
% Text Node
\draw (473.83,121.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 1$};
% Text Node
\draw (389.5,163.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 1$};
% Text Node
\draw (373.33,246.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 2$};
% Text Node
\draw (327,207.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 2$};
% Text Node
\draw (397,193.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 3$};
% Text Node
\draw (328.5,163.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 3$};
% Text Node
\draw (424.33,191) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 9$};
% Text Node
\draw (452,156.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 4$};
% Text Node
\draw (446.5,185.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 5$};
% Text Node
\draw (412.17,121.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 6$};
% Text Node
\draw (416.83,244.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 4$};
% Text Node
\draw (507.57,185.27) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{17.59pt}\setlength\topsep{0pt}
\textcolor[rgb]{0.29,0.56,0.89}{$\displaystyle p_{S}( u)$}
\end{minipage}};
% Text Node
\draw (295.75,190.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle a_{1}$};
% Text Node
\draw (307.47,127.01) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 45; green, 127; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle ball( u,A,S)$};


\end{tikzpicture}




\caption{\label{fig:ballexample} The ball $ball \left(u,A,S\right)$, where $A=\left\{ a_1,a_2,a_3\right\}$ and $S=\left\{s_1,s_2,s_3\right\}$. The pivot for $u$ is $p\left(u\right) = s_2$ with $\delta\left(u,S\right) = 5$.}
\end{figure}\vspace{-4mm}

==> Illustrations/Balls/inneredgesexample.tex <==
\begin{figure}[H]
\centering
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da87840787155437] 
\draw [color={rgb, 255:red, 13; green, 113; blue, 228 }  ,draw opacity=1 ]   (315.01,190.03) -- (361.51,163.03) ;
%Straight Lines [id:da052344792013143016] 
\draw [color={rgb, 255:red, 13; green, 113; blue, 228 }  ,draw opacity=1 ]   (315.01,190.03) -- (359.01,226.7) ;
%Straight Lines [id:da704512876406874] 
\draw [color={rgb, 255:red, 13; green, 113; blue, 228 }  ,draw opacity=1 ]   (359.01,226.7) -- (401.03,264.5) ;
%Straight Lines [id:da2529965611042688] 
\draw [color={rgb, 255:red, 13; green, 113; blue, 228 }  ,draw opacity=1 ]   (359.01,226.7) -- (435.03,227) ;
%Straight Lines [id:da038558601052662844] 
\draw [color={rgb, 255:red, 13; green, 113; blue, 228 }  ,draw opacity=1 ]   (401.03,264.5) -- (435.03,227) ;
%Straight Lines [id:da1453158167020543] 
\draw [color={rgb, 255:red, 13; green, 113; blue, 228 }  ,draw opacity=1 ]   (360.01,225.7) -- (434.53,164.5) ;
%Straight Lines [id:da8496894787108054] 
\draw [color={rgb, 255:red, 13; green, 113; blue, 228 }  ,draw opacity=1 ]   (434.53,164.5) -- (435.03,223) ;
%Straight Lines [id:da15583751877941343] 
\draw    (435.78,165.83) -- (472.03,201.5) ;
%Straight Lines [id:da6954206584025682] 
\draw    (438.53,162.5) -- (472.53,147.5) ;
%Straight Lines [id:da9064565291303313] 
\draw    (472.53,143.5) -- (472.28,111.17) ;
%Straight Lines [id:da53256747981667] 
\draw    (364.51,161.03) -- (468.85,113.37) ;
%Straight Lines [id:da35419788722237744] 
\draw [color={rgb, 255:red, 13; green, 113; blue, 228 }  ,draw opacity=1 ]   (365.51,163.03) -- (434.53,163.5) ;
%Shape: Circle [id:dp31720811305789964] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (357.51,163.03) .. controls (357.51,160.82) and (359.3,159.03) .. (361.51,159.03) .. controls (363.72,159.03) and (365.51,160.82) .. (365.51,163.03) .. controls (365.51,165.24) and (363.72,167.03) .. (361.51,167.03) .. controls (359.3,167.03) and (357.51,165.24) .. (357.51,163.03) -- cycle ;
%Shape: Circle [id:dp5265937509664673] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (355.01,226.7) .. controls (355.01,224.49) and (356.8,222.7) .. (359.01,222.7) .. controls (361.22,222.7) and (363.01,224.49) .. (363.01,226.7) .. controls (363.01,228.91) and (361.22,230.7) .. (359.01,230.7) .. controls (356.8,230.7) and (355.01,228.91) .. (355.01,226.7) -- cycle ;
%Shape: Circle [id:dp24609937249348568] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (311.01,190.03) .. controls (311.01,187.82) and (312.8,186.03) .. (315.01,186.03) .. controls (317.22,186.03) and (319.01,187.82) .. (319.01,190.03) .. controls (319.01,192.24) and (317.22,194.03) .. (315.01,194.03) .. controls (312.8,194.03) and (311.01,192.24) .. (311.01,190.03) -- cycle ;
%Shape: Circle [id:dp9874523059430802] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (430.53,163.5) .. controls (430.53,161.29) and (432.32,159.5) .. (434.53,159.5) .. controls (436.74,159.5) and (438.53,161.29) .. (438.53,163.5) .. controls (438.53,165.71) and (436.74,167.5) .. (434.53,167.5) .. controls (432.32,167.5) and (430.53,165.71) .. (430.53,163.5) -- cycle ;
%Shape: Circle [id:dp8586237542464736] 
\draw  [color={rgb, 255:red, 126; green, 211; blue, 33 }  ,draw opacity=1 ][fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (468.28,111.17) .. controls (468.28,108.96) and (470.07,107.17) .. (472.28,107.17) .. controls (474.49,107.17) and (476.28,108.96) .. (476.28,111.17) .. controls (476.28,113.38) and (474.49,115.17) .. (472.28,115.17) .. controls (470.07,115.17) and (468.28,113.38) .. (468.28,111.17) -- cycle ;
%Shape: Circle [id:dp8552923192966435] 
\draw  [color={rgb, 255:red, 126; green, 211; blue, 33 }  ,draw opacity=1 ][fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (468.53,147.5) .. controls (468.53,145.29) and (470.32,143.5) .. (472.53,143.5) .. controls (474.74,143.5) and (476.53,145.29) .. (476.53,147.5) .. controls (476.53,149.71) and (474.74,151.5) .. (472.53,151.5) .. controls (470.32,151.5) and (468.53,149.71) .. (468.53,147.5) -- cycle ;
%Shape: Circle [id:dp6801603655991799] 
\draw  [color={rgb, 255:red, 126; green, 211; blue, 33 }  ,draw opacity=1 ][fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (468.03,201.5) .. controls (468.03,199.29) and (469.82,197.5) .. (472.03,197.5) .. controls (474.24,197.5) and (476.03,199.29) .. (476.03,201.5) .. controls (476.03,203.71) and (474.24,205.5) .. (472.03,205.5) .. controls (469.82,205.5) and (468.03,203.71) .. (468.03,201.5) -- cycle ;
%Shape: Circle [id:dp7631537577629186] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (431.03,227) .. controls (431.03,224.79) and (432.82,223) .. (435.03,223) .. controls (437.24,223) and (439.03,224.79) .. (439.03,227) .. controls (439.03,229.21) and (437.24,231) .. (435.03,231) .. controls (432.82,231) and (431.03,229.21) .. (431.03,227) -- cycle ;
%Shape: Circle [id:dp4241349705641584] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (397.03,264.5) .. controls (397.03,262.29) and (398.82,260.5) .. (401.03,260.5) .. controls (403.24,260.5) and (405.03,262.29) .. (405.03,264.5) .. controls (405.03,266.71) and (403.24,268.5) .. (401.03,268.5) .. controls (398.82,268.5) and (397.03,266.71) .. (397.03,264.5) -- cycle ;

% Text Node
\draw (383.7,265) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle a_{3}$};
% Text Node
\draw (340.2,227) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle a_{2}$};
% Text Node
\draw (442.11,219.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle b_{2}$};
% Text Node
\draw (418.28,144.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle b_{1}$};
% Text Node
\draw (479.36,197) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 126; green, 211; blue, 33 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle s_{1}$};
% Text Node
\draw (479.36,107.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 126; green, 211; blue, 33 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle s_{3}$};
% Text Node
\draw (479.53,142.83) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 126; green, 211; blue, 33 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle s_{2}$};
% Text Node
\draw (357.53,170) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle u$};
% Text Node
\draw (394.28,213.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle 1$};
% Text Node
\draw (474.11,121.83) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 1$};
% Text Node
\draw (389.78,164) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle 1$};
% Text Node
\draw (373.61,246.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle 2$};
% Text Node
\draw (327.28,207.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle 2$};
% Text Node
\draw (397.28,193.83) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle 3$};
% Text Node
\draw (328.78,164.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle 3$};
% Text Node
\draw (424.61,191.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle 9$};
% Text Node
\draw (452.28,156.83) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 4$};
% Text Node
\draw (446.78,185.83) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 5$};
% Text Node
\draw (412.45,122.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 6$};
% Text Node
\draw (417.11,245) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle 4$};
% Text Node
\draw (296.03,190.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle a_{1}$};


\end{tikzpicture}

\caption{\label{fig:inneredgesexample} The inner-edges $E_{S}$ of all vertices $V$, in relation to $S$.}
\end{figure}

==> Illustrations/Balls/nearestexample.tex <==
\begin{figure}[H]
\centering

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Ellipse [id:dp6625860162276211] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=0.55 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.29 ] (301.45,234.55) .. controls (272.97,209.21) and (270.06,166) .. (294.94,138.04) .. controls (319.82,110.09) and (363.07,107.97) .. (391.55,133.32) .. controls (420.03,158.67) and (422.94,201.87) .. (398.06,229.83) .. controls (373.18,257.78) and (329.93,259.9) .. (301.45,234.55) -- cycle ;
%Straight Lines [id:da9412047664314018] 
\draw    (314.73,189.53) -- (361.23,162.53) ;
%Straight Lines [id:da5938656329561427] 
\draw    (314.73,189.53) -- (358.73,226.2) ;
%Straight Lines [id:da8588636129532099] 
\draw    (358.73,226.2) -- (434.75,226.5) ;
%Straight Lines [id:da7252060609228765] 
\draw    (359.73,225.2) -- (434.25,164) ;
%Straight Lines [id:da8370853051570586] 
\draw    (434.25,164) -- (434.75,222.5) ;
%Straight Lines [id:da23613900566954826] 
\draw    (198.43,200.43) -- (248.43,190.43) ;
%Straight Lines [id:da18676055033971273] 
\draw    (198.43,200.43) -- (255,153.67) ;
%Straight Lines [id:da2707706875989797] 
\draw    (252.43,186.43) -- (259,153.67) ;
%Straight Lines [id:da8302620780031216] 
\draw    (263.43,153.43) -- (357.23,162.53) ;
%Straight Lines [id:da8037223017346966] 
\draw    (365.23,162.53) -- (434.25,163) ;
%Shape: Circle [id:dp40608497322126125] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (357.23,162.53) .. controls (357.23,160.32) and (359.02,158.53) .. (361.23,158.53) .. controls (363.44,158.53) and (365.23,160.32) .. (365.23,162.53) .. controls (365.23,164.74) and (363.44,166.53) .. (361.23,166.53) .. controls (359.02,166.53) and (357.23,164.74) .. (357.23,162.53) -- cycle ;
%Shape: Circle [id:dp26827319251987447] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (354.73,226.2) .. controls (354.73,223.99) and (356.52,222.2) .. (358.73,222.2) .. controls (360.94,222.2) and (362.73,223.99) .. (362.73,226.2) .. controls (362.73,228.41) and (360.94,230.2) .. (358.73,230.2) .. controls (356.52,230.2) and (354.73,228.41) .. (354.73,226.2) -- cycle ;
%Shape: Circle [id:dp9709647852196648] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (310.73,189.53) .. controls (310.73,187.32) and (312.52,185.53) .. (314.73,185.53) .. controls (316.94,185.53) and (318.73,187.32) .. (318.73,189.53) .. controls (318.73,191.74) and (316.94,193.53) .. (314.73,193.53) .. controls (312.52,193.53) and (310.73,191.74) .. (310.73,189.53) -- cycle ;
%Shape: Circle [id:dp5706248374556] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (430.25,163) .. controls (430.25,160.79) and (432.04,159) .. (434.25,159) .. controls (436.46,159) and (438.25,160.79) .. (438.25,163) .. controls (438.25,165.21) and (436.46,167) .. (434.25,167) .. controls (432.04,167) and (430.25,165.21) .. (430.25,163) -- cycle ;
%Shape: Circle [id:dp6661137907917287] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (255,153.67) .. controls (255,151.46) and (256.79,149.67) .. (259,149.67) .. controls (261.21,149.67) and (263,151.46) .. (263,153.67) .. controls (263,155.88) and (261.21,157.67) .. (259,157.67) .. controls (256.79,157.67) and (255,155.88) .. (255,153.67) -- cycle ;
%Shape: Circle [id:dp1158857638153572] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (248.43,190.43) .. controls (248.43,188.22) and (250.22,186.43) .. (252.43,186.43) .. controls (254.64,186.43) and (256.43,188.22) .. (256.43,190.43) .. controls (256.43,192.64) and (254.64,194.43) .. (252.43,194.43) .. controls (250.22,194.43) and (248.43,192.64) .. (248.43,190.43) -- cycle ;
%Shape: Circle [id:dp7673589811197465] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (194.43,200.43) .. controls (194.43,198.22) and (196.22,196.43) .. (198.43,196.43) .. controls (200.64,196.43) and (202.43,198.22) .. (202.43,200.43) .. controls (202.43,202.64) and (200.64,204.43) .. (198.43,204.43) .. controls (196.22,204.43) and (194.43,202.64) .. (194.43,200.43) -- cycle ;
%Shape: Circle [id:dp5265818224073935] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (430.75,226.5) .. controls (430.75,224.29) and (432.54,222.5) .. (434.75,222.5) .. controls (436.96,222.5) and (438.75,224.29) .. (438.75,226.5) .. controls (438.75,228.71) and (436.96,230.5) .. (434.75,230.5) .. controls (432.54,230.5) and (430.75,228.71) .. (430.75,226.5) -- cycle ;
%Straight Lines [id:da295580442805107] 
\draw    (248.43,190.43) -- (314.73,189.53) ;

% Text Node
\draw (339.92,226.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle a_{2}$};
% Text Node
\draw (443.83,219.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle b_{2}$};
% Text Node
\draw (443,155) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle b_{1}$};
% Text Node
\draw (192.08,205.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle a_{3}$};
% Text Node
\draw (254.08,132.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle b_{3}$};
% Text Node
\draw (247.51,196.43) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle b_{4}$};
% Text Node
\draw (357.25,169.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle u$};
% Text Node
\draw (397,213) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 1$};
% Text Node
\draw (275.83,193.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 1$};
% Text Node
\draw (389.5,163.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 1$};
% Text Node
\draw (327,207.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 5$};
% Text Node
\draw (398,193.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 1$};
% Text Node
\draw (328.5,163.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 5$};
% Text Node
\draw (424.33,191) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 9$};
% Text Node
\draw (221,159.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 5$};
% Text Node
\draw (223.17,198.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 6$};
% Text Node
\draw (295.75,190.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle a_{1}$};
% Text Node
\draw (307.47,127.01) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 45; green, 127; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle \Gamma ( u,A,2)$};
% Text Node
\draw (295.94,142.04) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 1$};
% Text Node
\draw (260.17,165.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 1$};


\end{tikzpicture}






\caption{\label{fig:nearestexample} The set $\Gamma \paren{u,A,2}$, where $A=\left\{ a_1,a_2,a_3\right\}$.}
\end{figure}\vspace{-2mm}
